Human-centric light sensing and estimation from RGBD images: The invisible light switch

Lighting design in indoor environments is of primary importance for at least two reasons: 1) people should perceive an adequate light; 2) an effective lighting design means consistent energy saving. We present the Invisible Light Switch (ILS) to address both aspects. ILS dynamically adjusts the room illumination level to save energy while maintaining constant the light level perception of the users. So the energy saving is invisible to them. Our proposed ILS leverages a radiosity model to estimate the light level which is perceived by a person within an indoor environment, taking into account the person position and her/his viewing frustum (head pose). ILS may therefore dim those luminaires, which are not seen by the user, resulting in an effective energy saving, especially in large open offices (where light may otherwise be ON everywhere for a single person). To quantify the system performance, we have collected a new dataset where people wear luxmeter devices while working in office rooms. The luxmeters measure the amount of light (in Lux) reaching the people gaze, which we consider a proxy to their illumination level perception. Our initial results are promising: in a room with 8 LED luminaires, the energy consumption in a day may be reduced from 18585 to 6206 watts with ILS (currently needing 1560 watts for operations). While doing so, the drop in perceived lighting decreases by just 200 lux, a value considered negligible when the original illumination level is above 1200 lux, as is normally the case in offices.

==> sections/Abstract_backup.tex <==
\begin{abstract} \label{sec:abstract}
Lighting design in indoor environments is of primary importance for at least two reasons: 1) people should perceive an adequate light; 2) an effective lighting design means consistent energy saving.
We present the "Invisible Light Switch" (ILS), a framework which considers both the aspects. Thus, dynamically adjusting the illumination level so that to save energy and let the user being unaware of this with the impression of a stable illumination. %ILS builds upon our recent result, that is we are able to estimate the light in a room with multiple dimmable luminaries using a single RGB-d camera. 
ILS builds upon a novel system which is capable of estimating the light level perceived by a person independently of her position and motion in the room, thanks to robust radiosity modeling, human detection and head pose estimation. This in turn allows to dim down some luminaries as long as this does not change the human perception, resulting in a transparent but effective energy saving. A novel dataset has been created, where people wearing luxmeters do wander in a room and record the light level, mimicking in a realistic fashion the human perception. This unlocks the unprecedented possibility of quantitatively testing this scenario. The results are promising: in a single room illuminated with 8 LED luminaires, the energy expense in a day is 18585.6 watts . ILS, which needs 1560 watts to function, allows to lower down the total amount to 6206.4 watts in the most aggressive mode, causing a total 200 lux max of negative variation reaching to the user, which is shown to be not perceivable by the human when the initial illumination is 1200 lux.% (the standard ISO level for normal drawing work).




%https://www.noao.edu/education/QLTkit/ACTIVITY_Documents/Safety/LightLevels_outdoor+indoor.pdf






\iffalse

Human activity recognition and forecasting together with the lighting ambiance can be used as a primary cue for scene understanding. Acquiring details from the scene has vast applications in different fields such as computer vision, robotics and more recently smart lighting. Measuring and adjusting the indoor illumination and its changes over time is important in quality living and working indoor environments as well as for energy efficiency and power saving solutions. Lighting may improve the quality of life of people, a better lighting may help their productivity at work, while it may allow them to have a better relaxation at night and all this within a power efficiency framework.
% This work brings together advanced research in computer vision and the most modern technology in lighting. The goal of this work is to eliminate the need for any switches for lighting, which means that each person in the office perceives the entire office as “all lit”, while lights, which are not visible by the person, are switched off by the system. This can be achieved by combining lighting with presence detection and smart light control.
% Measuring the indoor illumination and its changes over time is important in quality living and working indoor environments. The effects of the spatial lighting on the human behaviour, the working routine and social activities has been thoroughly proven in the literature.
In this work we propose a complete pipeline for measuring both the spatial and the individual human perceived light automatically based on a camera-aided solution and using this information for showing how this could be used for a more power efficient lighting management solutions.
% We first estimate the spatial illumination as a general guideline of the ambient illumination of the room based on an advanced global illumination modeling technique, thereafter we detect the visible people within the camera's FOV and we extract the view frustum information of each individual. We then use the view frustum information in order to orient each individual person within the space so that to measure the light perceived from their location and model it in regards to the specific ego-perception of the total ambient light. 
We show that having the knowledge for both the total ambient light estimation as well as the individual light perceived from each person in the environment we can apply smart lighting applications related to activation/deactivation of unnecessary light sources providing a full-lit (optimally) feeling while it is minimally lit (invisible switch), adjusting the luminaires for keeping adequate light levels to personalized activities or light ISO standards. 
In that way this work we open a new applicability where the illumination modeling can be turned into an interactive process, allowing for real-time modifications and immediate feedback on the spatial illumination of a scene over time coupled with the personalized preferences.
\fi
%Selling idea is to set the baseline about whether such an approach is sufficient for modeling the human light perception together with the overall spatial illumination of the scene in real conditions with a camera-aided only input, so far only artificial based solutions {\color{blue}\url{https://faculty.washington.edu/inanici/Publications/InaniciNavvab.pdf}}\\  


% \begin{itemize}
% \item we estimate the light perceived by each human, the specific ego-perception of ambient lighting
% \item Application to power-saving, switching off the unnecessary.
% \item Application to personalized light level, set the received light to constant, everywhere the person sits and moves. (This is not a real-time implementation. This is rather applied to each frame.)
% \end{itemize}
\end{abstract}


